Fairness and Efficiency in Online Class Matching

The online bipartite matching problem, extensively studied in the literature, deals with the allocation of online arriving vertices (items) to a predetermined set of offline vertices (agents). However, little attention has been given to the concept of class fairness, where agents are categorized into different classes, and the matching algorithm must ensure equitable distribution across these classes. We here focus on randomized algorithms for the fair matching of indivisible items, subject to various definitions of fairness. Our main contribution is the first (randomized) non-wasteful algorithm that simultaneously achieves a $1/2$ approximation to class envy-freeness (CEF) while simultaneously ensuring an equivalent approximation to the class proportionality (CPROP) and utilitarian social welfare (USW) objectives. We supplement this result by demonstrating that no non-wasteful algorithm can achieve an $\alpha$-CEF guarantee for $\alpha > 0.761$. In a similar vein, we provide a novel input instance for deterministic divisible matching that demonstrates a nearly tight CEF approximation. Lastly, we define the ``price of fairness,'' which represents the trade-off between optimal and fair matching. We demonstrate that increasing the level of fairness in the approximation of the solution leads to a decrease in the objective of maximizing USW, following an inverse proportionality relationship.

==> Sections/trash.tex <==
\begin{theorem}[Adaptive adversary]
    For any $\eps>0$, there exists a problem instance such that no (possibly randomized) online algorithm with $1/2$-CEF can achieve USW larger than $1/2+\eps$.
\end{theorem}
\suho{all the results need to be verified / revised to be formal. todo: change the notation to be consistent with $V_i$ etc.}
Suppose that an algorithm is $1/2$-CEF.
Consider $k$ classes.
Class $1$ to $k-1$ have four agents.
Class $k$ have $2k+2$ agents.
$4k$ items arrive.
First $2k+2$ items have edges to all the agents.
Let $C_i(t)$ be a random variable that indicates how much item is allocated to class $i$ at the end of round $t$.

Let $\tau = 2k+2$.
We first claim that $\Ex{\sum_{i=1}^{k-1}C_i(\tau)} \ge 2k-2$.
Suppose not, i.e., $\Ex{\sum_{i=1}^{k-1}C_i(\tau)} < 2k-2$.
Then, obviously we have $\Ex{C_k(\tau)} \ge 4$.
Note further that there exists $i \in [k-1]$ such that $\Ex{C_i(\tau} < 2$.
This contradicts $1/2$-CEF at round $k+1$ since $\Ex{C_k(\tau)} \ge 4 > 2 \cdot \Ex{C_i(\tau)}$.

% Furthermore, note that $\Ex{\sum_{i=1}^{k-1}C_i(\tau)} \ge 2k-2$ implies that $\Ex{C_i(\tau)} = 2$ for $i \in [k-1]$ since each class $i \in [k-1]$ only have two agents so that the realization of $C_i(\tau)$ cannot exceed $2$.

Now suppose that the remaining $2k-2$ items arrive where each item have edges to all the agents in class $k$, and only to the agent in class $1$ to $k-1$ who is allocated in the first $2k+2$ rounds.
\suho{our adaptive adversary can do this?}
Then, the algorithm cannot further match these items to any agent.
Hence, the overall expected utility of any $1/2$-CEF algorithm will be $2k+2$.
On the other hand, given the same graph structure, a maximum matching will be to allocate the first $2k+2$ items to class $k$, and the remaining $2k-2$ items to classes $1$ to $k-1$, respectively.
This results in USW of $4k$.
Thus, any $1/2$-CEF algorithm has at most $\frac{2k+2}{4k}$-USW.
By making $k$ sufficiently large, this implies that for any $\eps>0$, there exists a problem instance such that any $1/2$-CEF algorithm cannot be better than $1/2+\eps$-USW.
\suho{$\eps$ here in fact depends on the problem parameter $k$.}

% By pigeonhole principle, at each realization of the first $k+1$ rounds, there exists a class which receives at least two items.



\begin{theorem}
    Parameterizing the above theorem.
\end{theorem}
\suho{I think we may parameterize the above theorem as follows. 
For any $\alpha \in (0,1)$, choose a sufficiently close rational approximation $\alpha = p/q$ for two coprimes $p$ and $q$ such that $q > p$.
Construct similar instance as above, but classes $1$ to $k-1$ have $q$ agents, and class $k$ has $q+p(k-1)$ agents.
Analogous analysis would imply that any online $\alpha$-CEF algorithm cannot do better than $\frac{1}{2} + \frac{1}{2+4\alpha(k-1)}$-USW.
This subsumes the above result.
Q: if we set $\alpha$ to be any value and let $k$ increase, then this implies that any $\eps$-CEF cannot guarantee better than $1/2+\eps'$-USW for some $\eps = f(\eps', k)$. Does it make sense? Probably this happens because $\eps$ actually depends on $k$, but I just regard it as some constants.} \ms{is there a type on this last statement? Do you meant $1/2 + \eps$-CEF? The result does make sense yes subject to the stronger adaptive adversary. I imagine we can modify the construction to be non-adaptive with a more careful item arrival sequence}
